Converting the Point of View of Messages Spoken to Virtual Assistants

Virtual Assistants can be quite literal at times. If the user says "tell Bob I love him," most virtual assistants will extract the message "I love him" and send it to the user's contact named Bob, rather than properly converting the message to "I love you." We designed a system to allow virtual assistants to take a voice message from one user, convert the point of view of the message, and then deliver the result to its target user. We developed a rule-based model, which integrates a linear text classification model, part-of-speech tagging, and constituency parsing with rule-based transformation methods. We also investigated Neural Machine Translation (NMT) approaches, including LSTMs, CopyNet, and T5. We explored 5 metrics to gauge both naturalness and faithfulness automatically, and we chose to use BLEU plus METEOR for faithfulness and relative perplexity using a separately trained language model (GPT) for naturalness. Transformer-Copynet and T5 performed similarly on faithfulness metrics, with T5 achieving slight edge, a BLEU score of 63.8 and a METEOR score of 83.0. CopyNet was the most natural, with a relative perplexity of 1.59. CopyNet also has 37 times fewer parameters than T5. We have publicly released our dataset, which is composed of 46,565 crowd-sourced samples.

==> metrics.tex <==
\section{Evaluation Metrics}\label{metrics}

Ideas are borrowed from paper Alexa, do you answer naturally: Automatic Evaluation of Answer Wording Without a Human Reference Set by Ye Tian et al.
The paper evaluates Alexa's output by adopting AQuA (Answer Quality Assessment) process on a 1-4 scale, identifies the 4 major wording problems, and creates training data for a binary classification to target area of improvements for Alexa (score 4 non-target, score 1-3 is target):

\begin{itemize}
\item Not a sentence: a word, phrase, or collection of words and phrases without a finite verb, rather than a sentence,
\item Phrasing: an answer not naturally phrased as a native-speaker human would speak it,
\item Grammatical error: an answer containing, for example, missing or excessive use of particles; agreement errors; tense errors; incorrect use of pronouns or prepositions, and
\item Semantically bad: an answer that is semantically empty or does not make sense.
\end{itemize}


